Convergence Analysis of Proximal Gradient with Momentum for Nonconvex Optimization

In many modern machine learning applications, structures of underlying mathematical models often yield nonconvex optimization problems. Due to the intractability of nonconvexity, there is a rising need to develop efficient methods for solving general nonconvex problems with certain performance guarantee. In this work, we investigate the accelerated proximal gradient method for nonconvex programming (APGnc). The method compares between a usual proximal gradient step and a linear extrapolation step, and accepts the one that has a lower function value to achieve a monotonic decrease. In specific, under a general nonsmooth and nonconvex setting, we provide a rigorous argument to show that the limit points of the sequence generated by APGnc are critical points of the objective function. Then, by exploiting the Kurdyka-{\L}ojasiewicz (\KL) property for a broad class of functions, we establish the linear and sub-linear convergence rates of the function value sequence generated by APGnc. We further propose a stochastic variance reduced APGnc (SVRG-APGnc), and establish its linear convergence under a special case of the \KL property. We also extend the analysis to the inexact version of these methods and develop an adaptive momentum strategy that improves the numerical performance.

==> svrg-exact.tex <==
\section{Proof of \Cref{thm: svrg}}\label{sec: thm: svrg}
We first define the following quantities for the convenience of the proof.
\begin{align}
&c_{t}=c_{t+1}(1+\tfrac{1}{m})+\tfrac{\eta L^2}{2},\ \ c_m=0,\label{eq: c_t}\\
&R_k^{t} \coloneqq \Ebb\left[F(\xb_k^{t})+c_t\|\xb_k^{t}-\xb_k^0\|^2\right], \\
&\bar{\xb}^{t+1}_k=\prox{\eta g}(\xb^t_k-\eta\nabla f(\xb^t_k)).\label{eq: ref}
\end{align}
	Note that $\bar{\xb}_k^{t+1}$ is a reference sequence introduced for the convenience of analysis, and is not being computed in the implementation of the algorithm.
	Then it has been shown in the proof of Theorem 5 of \cite{NIPS2016_6116} that
	\begin{align}\label{reddi}
	R_k^{t+1} \le R_k^t+\left(L-\tfrac{1}{2\eta}\right)\Ebb\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right].
	\end{align}

	Telescoping \cref{reddi} over $t$ from $t=1$ to $t=m-1$, we obtain
	\begin{align}
	\Ebb[F(\xb_k^{m})] \le \Ebb\left[F(\bar{\xb}_k^1)+c_1\|\bar{\xb}^1_k-\xb_k^0\|^2+\sum\limits_{t=1}^{m-1}\left(L-\tfrac{1}{2\eta}\right)\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right]. \label{eq: reddi_tele}
	\end{align}
Following from \cref{eq: c_t}, a simple induction shows that $c_t\le \eta L^2m$. Setting $\eta < \frac{1}{2L}$ and recalling that $F(\yb_k)\le F(\xb_{k-1}^m)$.,  \cref{eq: reddi_tele} further implies that
	\begin{align}\label{c1}
	\Ebb[F(\yb_{k+1})]\le	\Ebb[F(\xb_k^{m})] \le \Ebb[F(\bar{\xb}^1_k)]+\eta L^2m\Ebb[\|\bar{\xb}^1_k-\xb^0_k\|^2].
	\end{align}
	Now telescoping \cref{reddi} again over $t$ from $t=0$ to $t=m-1$ and applying \cref{c1}, we obtain
	\begin{align}\label{nonincreasing}
	\Ebb[F(\xb^{m}_k)]\le \Ebb[F(\yb_k)]+\sum\limits^{m-1}_{t=0}(L-\tfrac{1}{2\eta})\Ebb\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right].
	\end{align}
	Combining all the above facts, we conclude that for $\eta < \frac{1}{2L}$
	\begin{align}
	\Ebb[F(\yb_k)] \le \Ebb[F(\yb_{k-1})]\le \ldots \le F(\yb_{0}).
	\end{align}
	
%	It is assumed that $F$ is coersive, and then $\{E[F(\yb_{k})]\}$ is bounded. Thus, $\{E[F(\yb_{k})]\}$ has limit points. As $\{E[F(\yb_{k})]\}$ is nonincreasing, $\{E[F(\yb_{k})]\}$ has the same value $F^\ast$ at all the limit points.
%	
%	Since we have
%	\begin{align}
%	\sum\limits^{m-1}_{t=0}(\frac{1}{2\eta}-L)E\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right]	\le
%	E[F(\xb^{m}_k)]\le E[F(\yb_k)]-E[F(\yb_{k+1})],
%	\end{align}
%	we can add and telescope from $k=0$ to $\infty$ and obtain
%	\begin{align}
%	\sum\limits_{k=0}^{\infty}	\sum\limits^{m-1}_{t=0}(\frac{1}{2\eta}-L)E\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right] \le F(\yb_0)-F^\ast \le \infty.
%	\end{align}
%	Hence, $\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2 \rightarrow 0$ as $k\rightarrow \infty$. Let $t=0$ and we have $\|\bar{\xb}_k^{1}-\yb_k\|^2\rightarrow 0$ as $k\rightarrow \infty$.
%	
%	From  proximal mapping, we get
%	\begin{align}
%	\bar{\xb}_k^{1}=\argmin\limits_\xb \langle \nabla f(\yb_k), \xb-\yb_k \rangle+\frac{1}{2\eta}\|\xb-\yb_k\|^2+g(\xb),
%	\end{align}
%	and the optimality condition leads to
%	\begin{align}
%	\zero \in \nabla f(\yb_k)+\frac{1}{\eta} (\bar{\xb}^1_k-\yb_k)+\partial g(\bar{\xb}^1_k).
%	\end{align}
%	Thus, it can be shown that
%	\begin{align}
%	\nabla f(\bar{\xb}^1_k)-\nabla f(\yb_k)-\frac{1}{\eta}(\bar{\xb}^1_k-\yb_k) \in F(\bar{\xb}^1_k).
%	\end{align}
%	According to Lipschitz condition, we can obtain
%	\begin{align}
%	\|\nabla f(\bar{\xb}^1_k)-\nabla f(\yb_k)-\frac{1}{\eta}(\bar{\xb}^1_k-\yb_k)\| \le (L+\frac{1}{\eta})\|\bar{\xb}^1_k-\yb_k\|\rightarrow 0
%	\end{align}
%	as $k\rightarrow \infty$.
%	Therefore, we can have
%	\begin{align}
%	\lim\limits_{k\rightarrow \infty}\bar{\xb}^1_k=\lim\limits_{k\rightarrow \infty} \yb_k \triangleq y^\ast,\ \zero \in \partial F(y^\ast),
%	\end{align}
%	where $y^\ast$ is a limit point of the sequence $\{E[F(\yb_{k})]\}$, which is then also an optimal point.
	
	Since $\Ebb [F(\cdot)]$ is bounded below, $\Ebb[ F(\yb_k)]$ decreases to a finite limit, say, $F^*$. Define $r_k=\Ebb\left[ F(\yb_k)-F^\ast\right] $, and assume $r_k >0$ for all $k$ (since otherwise $r_k = 0$ and the algorithm terminates). Applying the \KL property with $\theta=1/2$, we obtain
	\begin{align}
	\tfrac{1}{c} (F(\xb)-F^\ast)^{\frac{1}{2}} \le \dist_{\partial F(\xb)} (\zero).
	\end{align}
	Setting $\xb=\bar{\xb}_k^1$, we further obtain
	\begin{align}
	\tfrac{1}{c^2} (F(\bar{\xb}_k^1)-F^\ast) \le \dist_{\partial F(\bar{\xb}^1_k)}^2 (\zero) \le \left(L+\tfrac{1}{\eta}\right)^2\|\bar{\xb}^1_k-\yb_k\|^2,
	\end{align}
	where the last inequality is due to \cref{eq: ref}.
	Taking expectation over both sides and using \cref{c1}, we obtain
	\begin{align}
	\tfrac{1}{c^2}	\Ebb[F(\xb_k^m)-F^\ast]-\tfrac{\eta L^2 m}{c^2}\Ebb\left[\|\bar{\xb}_k^1-\xb_k^0\|^2\right] \le  \left(L+\tfrac{1}{\eta}\right)^2\Ebb\left[\|\bar{\xb}^1_k-\yb_k\|^2\right].
	\end{align}
	Noting that $\xb_k^0=\yb_k$ and $\Ebb F(\yb_{k+1})	\le	\Ebb F(\xb_k^m)$, we then rearrange the above inequality and obtain
	\begin{align}
	\tfrac{1}{c^2}	\Ebb[F(\yb_{k+1})-F^\ast]	\le	\tfrac{1}{c^2}	\Ebb[F(\xb_k^m)-F^\ast] &\le \left[\left(L+\tfrac{1}{\eta}\right)^2+\tfrac{\eta L^2 m}{c^2}\right]\Ebb\left[\|\bar{\xb}^1_k-\yb_k\|^2\right]\\
	&\le \tfrac{\left(L+\frac{1}{\eta}\right)^2+\frac{\eta L^2 m}{c^2}}{\frac{1}{2\eta}-L}\left(\Ebb[F(\yb_k)]-E[F(\yb_{k+1})]\right) ,
	\end{align}
	which can be further rewritten as
	\begin{align}
	r_{k+1} \le d \left(r_k-r_{k+1}\right), 
	\end{align}
where $d=\tfrac{c^2\left(L+\frac{1}{\eta}\right)^2+{\eta L^2 m}}{\frac{1}{2\eta}-L}$. Then a simple induction yields that
	\begin{align}
	r_{k+1} \le \left(\tfrac{d}{d+1}\right)^{k+1}\left(F(\yb_0)-F^\ast\right).
	\end{align} 

==> svrg-inexact.tex <==
\section{Proof of \Cref{thm: svrg_inexact}}
We first introduce some auxiliary lemmas.
	\begin{lemma}\label{lemma1}
		Consider the convex function $g$ and $\xb,\yb \in \RR^d$ such that $\yb=\prox{\eta g}^\epsilon (\xb)$ for some $\epsilon >0$. Then, there exists $\|\ib\| \le \sqrt{2\eta \epsilon}$ that satisfies the following inequality for all $\zb\in \RR^d$.
		\begin{align}
		g(\yb)+\tfrac{1}{2\eta}\|\yb-\xb\|^2 \le g(\zb)+\tfrac{1}{2\eta}\|\zb-\xb\|^2-\tfrac{1}{2\eta}\|\yb-\zb\|^2+\langle \yb-\zb,\tfrac{1}{\eta}\ib \rangle		+\epsilon.	
		\end{align}
	\end{lemma}
	\begin{proof}
		By Lemma 2 in \cite{inexact_pga}, there exists $\|\ib\| \le \sqrt{2\eta \epsilon}$ such that
		\begin{align}
		\tfrac{1}{\eta}\left(\xb-\yb-\ib\right) \in \partial_\epsilon g(\yb).
		\end{align}
		Then, the definition of $\epsilon$-subdifferential implies that
		\begin{align}
		g(\zb)-g(\yb) &\ge \langle \zb-\yb, \partial_\epsilon g(\yb)\rangle-\epsilon = \langle \zb-\yb, \tfrac{1}{\eta}\left(\xb-\yb-\ib\right)\rangle-\epsilon,~\forall~\zb \in \RR^d.
		\end{align}
		The desired result follows by rearranging the above inequality.
	\end{proof}
	\begin{lemma}\label{lemma2}
		Consider the convex function $g$ and $\xb,\yb, \db\in \RR^d$ such that $\yb=\prox{\eta g}^\epsilon(\xb-\eta \db)$ for some $\epsilon >0$. Then, there exists $\|\ib\| \le \sqrt{2\eta \epsilon}$ that satisfies the following inequality for all $\zb\in \RR^d$.
		\begin{align}
		g(\yb)=\langle \yb-\zb, \db -\tfrac{1}{\eta} \ib\rangle \le g(\zb)+ \tfrac{1}{2\eta} \left[\|\zb-\xb\|^2-\|\yb-\zb\|^2-\|\yb-\xb\|^2\right]+\epsilon.
		\end{align}
	\end{lemma}
	\begin{proof}
		By \Cref{lemma1}, we obtain the following inequality for all $\zb\in \RR^d$.
		\begin{align}
g(\yb) &+\langle \yb-\xb,\db\rangle +\tfrac{1}{2\eta}\|\yb-\xb\|^2+\frac{\eta}{2}\|\db\|^2 \nonumber \\
& \quad \le g(\zb)+\tfrac{1}{2\eta}\|\zb-\xb+\eta \db\|^2-\tfrac{1}{2\eta}\|\yb-\zb\|^2+\langle \yb-\zb,\tfrac{1}{\eta} \ib\rangle+\epsilon \nonumber \\
		&\quad = g(\zb)+\langle \zb-\xb, \db\rangle \tfrac{1}{2\eta}\|\zb-\xb\|^2+\tfrac{\eta}{2}\|\db\|^2-\tfrac{1}{2\eta}\|\yb-\zb\|^2+\langle \yb-\zb,\tfrac{1}{\eta} \ib \rangle+\epsilon.
		\end{align}
		The desired result follows by rearranging the above inequality.
	\end{proof}
	\begin{lemma}\label{lemma3}
		Consider the convex function $g$ and $\xb,\yb, \db\in \RR^d$ such that $\yb=\prox{\eta g}^\epsilon(\xb-\eta \db)$ for some $\epsilon >0$. Then, there exists $\|\ib\| \le \sqrt{2\eta \epsilon}$ that satisfies the following inequality for all $\zb\in \RR^d$.
		\begin{align}
		F(\yb)+\langle \yb-\zb,\db-\tfrac{1}{\eta} \ib-\nabla f(\xb) \rangle \le F(\zb)+\left(\tfrac{L}{2}-\tfrac{1}{2\eta}\right)\|\yb-\xb\|^2+\left(\tfrac{L}{2}+\tfrac{1}{2\eta}\right)\|\zb-\xb\|^2-\tfrac{1}{2\eta}\|\yb-\zb\|^2+\epsilon.
		\end{align}
		\begin{proof}
			By Lipschitz continuity of $\nabla f$, we obtain
			\begin{align}
			f(\yb) \le f(\xb)+\langle \nabla f(\xb),\yb-\xb \rangle +\tfrac{L}{2}\|\yb-\xb\|^2,\\
			f(\xb) \le f(\zb)+\langle \nabla f(\xb),\xb-\zb \rangle +\tfrac{L}{2}\|\xb-\zb\|^2.
			\end{align}
			Adding the above inequalities together yields
			\begin{align}
			f(\yb)\le f(\zb)+\langle \nabla f(\xb), \yb-\zb \rangle +\tfrac{L}{2}\left[\|\yb-\xb\|^2+\|\zb-\xb\|^2\right].
			\end{align}
			Combining with \Cref{lemma2}, we then obtain the desired result.
		\end{proof}
	\end{lemma}
	
	Recall the reference sequence $\bar{\xb}^{t+1}_k=\prox{\eta g}(\xb^t_k-\eta\nabla f(\xb^t_k))$.	
	Applying \Cref{lemma3} with $\epsilon=0$, $\yb=\bar{\xb}^{t+1}_k$, $\zb=\xb^t_k$, and $\db=\nabla f(\xb^t_k)$ and taking expectation on both sides, we obtain
	\begin{align}\label{24}
	\Ebb[F(\bar{\xb}^{t+1}_k)] \le \Ebb\left[F(\xb^t_k)+\left(\tfrac{L}{2}-\tfrac{1}{2\eta}\right)\|\bar{\xb}^{t+1}_k) - \xb^t_k\|^2-\tfrac{1}{2\eta}\|\bar{\xb}^{t+1}_k - \xb^t_k\|^2\right].
	\end{align}
	Similarly, applying \Cref{lemma3} with $\epsilon=\epsilon_k^t$, $\yb=\xb^{t+1}_{k}$, $\zb=\bar\xb^{t+1}_k$, $\db=\vb_k^t$ and taking expectation on both sides, we obtain
	\begin{align}\label{25}
	\Ebb[F({\xb}^{t+1}_k)] &\le \Ebb\left[F(\bar\xb^{t+1}_k)+\langle\xb^{t+1}_k-\bar{\xb}^{t+1}_k, \nabla f\left(\xb^t_k \right)-\vb_k^t+\tfrac{1}{\eta}\ib_k \rangle\right.\nonumber\\
	&\left.+\left(\tfrac{L}{2}-\tfrac{1}{2\eta}\right)\|{\xb}^{t+1}_k - \xb^t_k\|^2+\left(\tfrac{L}{2}+\tfrac{1}{2\eta}\right)\|\bar{\xb}^{t+1}_k - \xb^t_k\|^2-\tfrac{1}{2\eta}\|\bar{\xb}^{t+1}_k - \xb^{t+1}_k\|^2+\epsilon_k^t\right].
	\end{align}
	Adding \cref{24} and \cref{25} together yields
	\begin{align}\label{26}
	\Ebb[F({\xb}^{t+1}_k)] \le \Ebb\left[F(\xb^t_k)+\left({L}-\tfrac{1}{2\eta}\right)\|\bar{\xb}^{t+1}_k- \xb^t_k\|^2 +\left(\tfrac{L}{2}-\tfrac{1}{2\eta}\right)\|{\xb}^{t+1}_k - \xb^t_k\|^2-\tfrac{1}{2\eta}\|\bar{\xb}^{t+1}_k - \xb^{t+1}_k\|^2+T\right]
	\end{align}
	where $T=\langle\xb^{t+1}_k-\bar{\xb}^{t+1}_k, \nabla f\left(\xb^t_k \right)-\vb_k^t+\frac{\mathbf{i}_k}{\eta} \rangle+\epsilon_k^t$.
	Now we bound $\Ebb[T]$ as follows.
	\begin{align}
	\Ebb[T] &\le \tfrac{1}{2\eta} \Ebb\left[ \|\xb^{t+1}_k -  \xb^{t+1}_k \|^2\right]+\tfrac{\eta}{2}\Ebb\left[ \| \nabla f\left(\xb^t_k \right)-\vb_k^t+\tfrac{\mathbf{i}_k}{\eta}\|^2 \right] +\epsilon_k^t \\
	&\le 	\tfrac{1}{2\eta} \Ebb\left[ \|\xb^{t+1}_k -  \xb^{t+1}_k \|^2\right]+{\eta}\Ebb\left[ \| \nabla f\left(\xb^t_k \right)-\vb_k^t\|^2 \right] +\eta \Ebb\left[ \|\tfrac{\mathbf{i}_k}{\eta} \|^2\right]+\epsilon_k^t \\
	&\le \tfrac{1}{2\eta} \Ebb\left[ \|\xb^{t+1}_k -  \xb^{t+1}_k \|^2\right]+{\eta}\Ebb\left[ \| \nabla f\left(\xb^t_k \right)-\vb_k^t\|^2 \right] +3\epsilon_k^t.
	\end{align}
	By Lemma 3 of \cite{NIPS2016_6116}, it holds that $\Ebb\left[ \| \nabla f\left(\xb^t_k \right)-\vb_k^t\|^2 \right] \le L^2 \Ebb\left[ \|\xb^t_k- \xb^0_{k}\|^2\right].$ Combining with the above inequality,	
	we further obtain that
	\begin{align}
	\Ebb[T]\le \tfrac{1}{2\eta} \Ebb\left[ \|\xb^{t+1}_k -  \xb^{t+1}_k \|^2\right]+\eta L^2 \Ebb\left[ \|\xb^t_k- \xb^0_{k}\|^2\right]+3\epsilon_k^t.
	\end{align}
	Substituting the above result into \cref{26}, we obtain
	\begin{align}
	\Ebb[F({\xb}^{t+1}_k)] \le \Ebb\left[F(\xb^t_k)+\left({L}-\tfrac{1}{2\eta}\right)\|\bar{\xb}^{t+1}_k- \xb^t_k\|^2 +\left(\tfrac{L}{2}-\tfrac{1}{2\eta}\right)\|{\xb}^{t+1}_k - \xb^t_k\|^2+\eta L^2  \|\xb^t_k- \xb^0_{k}\|^2+3\epsilon_k^t\right].
	\end{align}
	Recalling that $R_k^{t} \coloneqq \Ebb\left[F(\xb_k^{t})+c_t\|\xb_k^{t}-\xb_k^0\|^2\right],$ where $	c_t=\eta L^2 \frac{(1+\beta)^{m-t}-1}{\beta}$
	with $\beta>0$.
	Then, we can upper bound $R_k^{t+1}$ as
	\begin{align}
	R_k^{t+1} =& \Ebb \left[ F(\xb^{t+1}_k) +c_{t+1}\|\xb^{t+1}_k-\xb^{t}_k+\xb^{t}_k-\xb^{0}_k\|^2\right]\\
	=&\Ebb \left[ F(\xb^{t+1}_k) +c_{t+1}\left( \|\xb^{t+1}_k-\xb^{t}_k\|^2+\|\xb^{t}_k-\xb^{0}_k\|^2+2\langle\xb^{t+1}_k-\xb^{t}_k,\xb^{t}_k-\xb^{0}_k \rangle\right) \right]\\
	\le & \Ebb\left[ F(\xb^{t+1}_k) +c_{t+1}\left(1+\tfrac{1}{\beta} \right) \|\xb^{t+1}_k-\xb^{t}_k\|^2+c_{t+1}\left(1+{\beta} \right)\|\xb^{t}_k-\xb^{0}_k\|^2  \right]\\
	\le & \Ebb\left[F(\xb^t_k)+\left({L}-\tfrac{1}{2\eta}\right)\|\bar{\xb}^{t+1}_k- \xb^t_k\|^2 +\left[c_{t+1}\left(1+\tfrac{1}{\beta} \right) +\tfrac{L}{2}-\tfrac{1}{2\eta}\right] \|{\xb}^{t+1}_k - \xb^t_k\|^2\right. \\&\left. +\left[ c_{t+1}\left(1+{\beta} \right)+\eta L^2\right]   \|\xb^t_k- \xb^0_{k}\|^2+3\epsilon_k^t\right].
	\end{align}
	
	Setting $\beta=1/m$ in $c_t$ and observe that
	\begin{align}
	c_t=\eta L^2 \tfrac{(1+\beta)^{m-t}-1}{\beta} =\eta L^2m\left( {(1+\beta)^{m-t}-1}\right) \le \eta L^2m\left( e-1\right) \le 2\eta L^2m,
	\end{align}
	which further implies that
	\begin{align}
	c_{t+1}\left(1+\tfrac{1}{\beta} \right)+ \tfrac{L}{2} \le  2\eta L^2m(1+m)\le 4\eta L^2m^2+ \tfrac{L}{2} =4\rho Lm^2+ \tfrac{L}{2} \le \tfrac{1}{2\eta}.
	\end{align}
	
	Also note that $c_t=c_{t+1}(1+\beta)+\eta L^2$. Collecting all these facts, $R_k^{t+1}$ can be further upper bounded by
	\begin{align}\label{reddi+error}
	R_k^{t+1} \le R_k^{t}+\Ebb\left[ \left({L}-\tfrac{1}{2\eta}\right)\|\bar{\xb}^{t+1}_k- \xb^t_k\|^2+3\epsilon_k^t \right].
	\end{align}
	
	
	
	Telescoping \cref{reddi+error} from $t=1$ to $t=m-1$, we obtain
	\begin{align}\label{c1+error}
	\Ebb[F(\xb_k^{m})] \le \Ebb\left[F(\bar{\xb}_k^1)+c_1\|\bar{\xb}^1_k-\xb_k^0\|^2+\sum\limits_{t=1}^{m-1}\left(L-\tfrac{1}{2\eta}\right)\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2+\sum\limits_{t=1}^{m-1} 3\epsilon_k^t\right].
	\end{align}
	
	Again, telescoping \cref{reddi+error} from $t=0$ to $t=m-1$ we obtain
	\begin{align}\label{nonincreasing+error}
	\Ebb[F(\yb_{k+1})]\le
	\Ebb[F(\xb^{m}_k)]\le \Ebb[F(\yb_k)]+\sum\limits^{m-1}_{t=0}(L-\tfrac{1}{2\eta})\Ebb\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right]+3\sum\limits_{t=0}^{m-1}\Ebb\left[  \epsilon_k^t\right].
	\end{align}
	
	Assume $\sum\limits^{m-1}_{t=0}\Ebb\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2 \right] >0$, because otherwise the algorithm is terminated. Assume that there exists $\alpha>0$ such that $3\sum\limits_{t=0}^{m-1}\Ebb\left[  \epsilon_k^t\right] \le \alpha \sum\limits^{m-1}_{t=0}\Ebb\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2 \right]$ and $\frac{1}{2\eta}-L-\alpha >0$. Then \cref{nonincreasing+error} further implies that
	\begin{align}
	\Ebb[F(\yb_{k+1})]\le
	\Ebb[F(\xb^{m}_k)]\le \Ebb[F(\yb_k)]+\sum\limits^{m-1}_{t=0}(L-\tfrac{1}{2\eta}+\alpha)\Ebb\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right].
	\end{align}
	That is, we have $\Ebb[F(\yb_k)] \le \Ebb[F(\yb_{k-1})]\le \ldots \le F(\yb_{0})$, and hence $\Ebb[F(\yb_k)] \downarrow F^*$.
%	It is assumed that $F$ is coersive, and then $\{E[F(\yb_{k})]\}$ is bounded. Thus, $\{E[F(\yb_{k})]\}$ has limit points. As $\{E[F(\yb_{k})]\}$ is nonincreasing, $\{E[F(\yb_{k})]\}$ has the same value $F^\ast$ at all the limit points.
%	
%	Since we have
%	\begin{align}
%	\sum\limits^{m-1}_{t=0}(\frac{1}{2\eta}-L-\alpha)E\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right]	\le
%	E[F(\xb^{m}_k)]\le E[F(\yb_k)]-E[F(\yb_{k+1})],
%	\end{align}
%	we can add and telescope from $k=0$ to $\infty$ and obtain
%	\begin{align}
%	\sum\limits_{k=0}^{\infty}	\sum\limits^{m-1}_{t=0}(\frac{1}{2\eta}-L-\alpha)E\left[\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right] \le F(\yb_0)-F^\ast \le \infty.
%	\end{align}
%	Hence, $\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2 \rightarrow 0$ as $k\rightarrow \infty$. Let $t=0$ and we have $\|\bar{\xb}_k^{1}-\yb_k\|^2\rightarrow 0$ as $k\rightarrow \infty$.
%	
%	From  proximal mapping, we get
%	\begin{align}
%	\bar{\xb}_k^{1}=\argmin\limits_\xb \langle \nabla f(\yb_k), \xb-\yb_k \rangle+\frac{1}{2\eta}\|\xb-\yb_k\|^2+g(\xb),
%	\end{align}
%	and the optimality condition leads to
%	\begin{align}
%	\zero \in \nabla f(\yb_k)+\frac{1}{\eta} (\bar{\xb}^1_k-\yb_k)+\partial g(\bar{\xb}^1_k).
%	\end{align}
%	Thus, it can be shown that
%	\begin{align}
%	\nabla f(\bar{\xb}^1_k)-\nabla f(\yb_k)-\frac{1}{\eta}(\bar{\xb}^1_k-\yb_k) \in F(\bar{\xb}^1_k).
%	\end{align}
%	According to Lipschitz condition, we can obtain
%	\begin{align}
%	\|\nabla f(\bar{\xb}^1_k)-\nabla f(\yb_k)-\frac{1}{\eta}(\bar{\xb}^1_k-\yb_k)\| \le (L+\frac{1}{\eta})\|\bar{\xb}^1_k-\yb_k\|\rightarrow 0
%	\end{align}
%	as $k\rightarrow \infty$.
%	Therefore, we can have
%	\begin{align}
%	\lim\limits_{k\rightarrow \infty}\bar{\xb}^1_k=\lim\limits_{k\rightarrow \infty} \yb_k \triangleq y^\ast,\ \zero \in \partial F(y^\ast),
%	\end{align}
%	where $y^\ast$ is a limit point of the sequence $\{E[F(\yb_{k})]\}$, which is then also an optimal point.
		We can further upper bound \cref{c1+error} as
	\begin{align}\label{m1+error}
	\Ebb[F(\xb_k^{m})] \le & \Ebb\left[F(\bar{\xb}_k^1)+c_1\|\bar{\xb}^1_k-\xb_k^0\|^2+\sum\limits_{t=1}^{m-1}\left(L-\tfrac{1}{2\eta}\right)\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2+\sum\limits_{t=1}^{m-1} 3\epsilon_k^t\right]\nonumber\\
	\le & E\left[F(\bar{\xb}_k^1)+c_1\|\bar{\xb}^1_k-\xb_k^0\|^2-\left(L-\tfrac{1}{2\eta}\right)\|\bar{\xb}^1_k-\xb_k^0\|^2+\sum\limits_{t=0}^{m-1}\left(L-\tfrac{1}{2\eta}\right)\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2+\sum\limits_{t=0}^{m-1} 3\epsilon_k^t\right]\nonumber\\
	\le & \Ebb\left[F(\bar{\xb}_k^1)+\left( c_1+\tfrac{1}{2\eta}\right) \|\bar{\xb}^1_k-\xb_k^0\|^2+\sum\limits_{t=0}^{m-1}\left(L-\tfrac{1}{2\eta}+\alpha\right)\|\bar{\xb}_k^{t+1}-{\xb}_k^t\|^2\right]\nonumber\\
	\le & \Ebb\left[ F(\bar{\xb}_k^1) \right]+\Ebb\left[ \left( 2\eta L^2m+\tfrac{1}{2\eta}\right) \|\bar{\xb}^1_k-\xb_k^0\|^2 \right].
	\end{align}
	
	Define $r_k=\Ebb\left[ F(\yb_k)-F^\ast\right] $, and suppose $r_k >0$ for all $k$ (otherwise the algorithm terminates in finite steps). Applying the \KL condition with $\theta=1/2$, we obtain
	\begin{align}
	\tfrac{1}{c} (F(\xb)-F^\ast)^{\frac{1}{2}} \le \dist_{\partial F(\xb)} (\zero).
	\end{align}
	Setting $\xb=\bar{\xb}_k^1$, we obtain
	\begin{align}
	\frac{1}{c^2} (F(\bar{\xb}_k^1)-F^\ast) \le \dist_{\partial F(\bar{\xb}^1_k)}^2 (\zero) \le \left(L+\tfrac{1}{\eta}\right)^2\|\bar{\xb}^1_k-\yb_k\|^2.
	\end{align}
	Taking expectation on both sides and using the result from \cref{m1+error}, we obtain
	\begin{align}
	\frac{1}{c^2}\Ebb[F(\xb_k^m)-F^\ast]-\tfrac{2\eta L^2 m+\frac{1}{2\eta}}{c^2}\Ebb\left[\|\bar{\xb_k}^1-\xb_k^0\|^2\right] \le  \left(L+\tfrac{1}{\eta}\right)^2 \Ebb\left[\|\bar{\xb}^1_k-\yb_k\|^2\right].
	\end{align}
	Note that $\xb_k^0=\yb_k$. Then rearranging the above inequality yields
	\begin{align}
	\tfrac{1}{c^2}	\Ebb[F(\yb_{k+1})-F^\ast]	\le	\frac{1}{c^2}	E[F(\xb_k^m)-F^\ast] &\le \left[\left(L+\tfrac{1}{\eta}\right)^2+\tfrac{2\eta L^2 m+\frac{1}{2\eta}}{c^2}\right]\Ebb\left[\|\bar{\xb}^1_k-\yb_k\|^2\right]\\&\le \tfrac{\left(L+\frac{1}{\eta}\right)^2+\frac{2\eta L^2 m+\frac{1}{2\eta}}{c^2}}{\frac{1}{2\eta}-L-\alpha}\left(\Ebb[F(\yb_k)]-\Ebb[F(\yb_{k+1})]\right) ,
	\end{align}
	which can be rewritten as $r_{k+1} \le d \left(r_k-r_{k+1}\right)$
	with $d=\tfrac{c^2\left(L+\frac{1}{\eta}\right)^2+{2\eta L^2 m+\frac{1}{2\eta}}}{\frac{1}{2\eta}-L-\alpha}$.
	Then, induction yields that
	\begin{align}
	r_{k+1} \le \frac{d}{d+1}r_k \le \left(\frac{d}{d+1}\right)^{k+1}\left(F(\yb_0)-F^\ast\right).
	\end{align}
	
